A Theory of How Pretraining Shapes Inductive Bias in Fine-Tuning

Pretraining and fine-tuning are central stages in modern machine learning systems. In practice, feature learning plays an important role across both stages: deep neural networks learn a broad range of useful features during pretraining and further refine those features during fine-tuning. However, an end-to-end theoretical understanding of how choices of initialization impact the ability to reuse and refine features during fine-tuning has remained elusive. Here we develop an analytical theory of the pretraining fine-tuning pipeline in diagonal linear networks, deriving exact expressions for the generalization error as a function of initialization parameters and task statistics. We find that different initialization choices place the network into four distinct fine-tuning regimes that are distinguished by their ability to support feature learning and reuse and therefore by the task statistics for which they are beneficial. In particular, a smaller initialization scale in earlier layers enables the network to both reuse and refine its features, leading to superior generalization on fine-tuning tasks that rely on a subset of pretraining features. We demonstrate empirically that the same initialization parameters impact generalization in ResNets trained on CIFAR-100 and SVHN as well as Transformers trained on modular arithmetic tasks. Overall, our results demonstrate an alytically how data and network initialization interact to shape fine-tuning generalization, highlighting an important role for the relative scale of initialization across different layers in enabling continued feature learning during fine-tuning.

==> ridge_regression.tex <==
\section{High-dimensional statistics of pretraining-specific regularization}

\subsection{Setup}
We consider a high-dimensional linear regression model with
\emph{coordinate-dependent regularization}. This coordinate-dependent regularization will correspond to the effect of pretraining on the different features.

Let
\begin{align}
&X \in \mathbb{R}^{n\times m}, 
\qquad 
\beta^* \in \mathbb{R}^m,
\qquad 
y \in \mathbb{R}^n ,\\
&X_{ij} \sim \mathcal{N}(0,1/n)\ \text{i.i.d.}, 
\qquad 
w \sim \mathcal{N}(0,\sigma_0^2 I_n),\\
&y = X\beta^* + w .
\end{align}

We then consider the asymptotic regime
\begin{align}
n,m \to \infty,
\qquad 
\frac{m}{n} \to \gamma_{FT} \in (0,\infty). \tag{4}
\end{align}

For each coordinate $j=1,\dots,m$, we associate a ground-truth coefficient $\beta_j^*$, and
a (possibly random) regularization function $f_j:\mathbb{R}\to\mathbb{R}\cup\{+\infty\}$. 

We assume that the pairs $(\beta_j^*,f_j)$ are i.i.d. across coordinates with the joint probability distribution
$P_{\beta,f}$:
\begin{align}
(\beta_j^*,f_j)_{j=1}^m \ \text{i.i.d.} \sim P_{\beta,f}. \tag{5}
\end{align}
Though this isn't necessary, we will then generally assume
\begin{equation}
    \mathbb{E}[\beta_j^*|f_j]=0.
\end{equation}
Given $\lambda>0$, we then define the estimator
\begin{align}
\hat\beta
:=
\arg\min_{\beta\in\mathbb{R}^m}
\left\{
\|y - X\beta\|_2^2
+
\lambda \sum_{j=1}^m f_j(\beta_j)
\right\}.
\end{align}
The joint distribution between $(\beta_j^*,f_j)$ formalizes that we may encode some knowledge about our ground-truth coefficients in the regularizer $f_j$. Put differently, we have a conditional distribution
\begin{equation}
    \beta_j^*|f_j.
\end{equation}
From a Bayesian perspective $f_j$ formalizes our assumptions about the distribution of $\beta_j$, i.e.
\begin{equation}
    p_{\beta|f}(\beta|f)=C^{-1}\exp(-\tau f(\beta)),
\end{equation}
where $\tau>0$ and $C$ is the normalization constant. Importantly, we also consider cases, however, where the conditional distribution does not match our regularization.

We then define the asymptotic per-coordinate estimation error
\begin{align}
\mathcal{E}_m
:=
\frac{1}{m}\,
\mathbb{E}\big\|\hat\beta - \beta^*\big\|_2^2 ,
\end{align}
where the expectation is taken over $(X,\beta^*,f,w)$. We will characterize
\begin{equation}
    \mathcal{E}:=\lim_{n\to\infty}\mathcal{E}_{m(n)}.
\end{equation}

\subsection{Ridge regression}
We start by developing an intuition in the ridge regression case:
\begin{equation}
    f_j(x):=\mu_jx^2.
\end{equation}
In this case, we denote the distribution over $\mu_j$ rather than $f_j$. We can then express the error in terms of a matrix product allowing us to subsequently characterize this error in terms of random matrix theory.
Let
\[
M := \mathrm{diag}(\mu_1,\dots,\mu_m).
\]

The estimator becomes
\[
\hat\beta
= \arg\min_{\beta\in\mathbb{R}^m}
\big\|y - X\beta\big\|_2^2 + \lambda\,\beta^\top M \beta,
\]
which admits the closed-form solution
\[
\hat\beta = (X^\top X + \lambda M)^{-1} X^\top y.
\]

Substituting the data model $y = X\beta^* + w$, we obtain
\[
\hat\beta - \beta^*
=
\big[(X^\top X + \lambda M)^{-1}X^\top X - I\big]\beta^*
\;+\;
(X^\top X + \lambda M)^{-1}X^\top w.
\]

Using the identity
\[
(X^\top X + \lambda M)^{-1}X^\top X - I
= -\lambda (X^\top X + \lambda M)^{-1} M,
\]
the estimation error decomposes as
\[
\hat\beta - \beta^*
=
-\lambda (X^\top X + \lambda M)^{-1} M \beta^*
\;+\;
(X^\top X + \lambda M)^{-1}X^\top w.
\]

This representation makes explicit that the estimation error is the sum of
\emph{(i)} a shrinkage term acting linearly on $\beta^*$ and
\emph{(ii)} a noise amplification term acting linearly on $w$.

Taking squared norms and expectations, the per-coordinate estimation error can be written as
\[
\mathcal{E}_m
=
\frac{\lambda^2}{m}\,
\mathbb{E}\!\left[
\beta^{*\top}
M (X^\top X + \lambda M)^{-2} M
\beta^*
\right]
+
\frac{\sigma_0^2}{m}\,
\mathbb{E}\!\left[
\mathrm{Tr}\!\left(
X^\top X (X^\top X + \lambda M)^{-2}
\right)
\right],
\]
where the cross term vanishes due to the independence of $\beta^*$ and $w$ and the
zero-mean assumption on the noise.

We express this expression using the resolvent $G_{\lambda}:=(X^\top X + \lambda M)^{-1}$ and the sample covariance matrix $\hat{\Sigma}:=X^TX$. The first expression evaluates to
\begin{equation}
    \mathbb{E}\!\left[
\beta^{*\top}
M (X^\top X + \lambda M)^{-2} M
\beta^*
\right]=\sum_{j=1}^m\mathbb{E}\!\left[\mu_j^2(G_\lambda)_{jj}^{2}\beta_j^2\right],
\end{equation}
where we get rid of the off-diagonal contributions because $\beta_i,\beta_j$ are independent and have zero expectation when conditioned on $M$. Defining
\begin{equation}
    q(\mu_j):=\mathbb{E}[\beta_j^2|\mu_j],
\end{equation}
we rewrite this as
\begin{equation}
    \mathbb{E}\!\left[
\beta^{*\top}
M (X^\top X + \lambda M)^{-2} M
\beta^*
\right]=\sum_{j=1}^m\mathbb{E}\!\left[(G_\lambda)_{jj}^{2}\mu_j^2q(\mu_j^2)\right].
\end{equation}
To solve this expression, we define $\tilde{X}:=XM^{-1/2}$ and
\begin{equation}
    \hat{\tilde{\Sigma}}:=\frac{1}{n}\tilde{X}^T\tilde{X},\quad
    Q(z):=(\hat{\tilde{\Sigma}}-zI)^{-1}, z\in\mathbb{C}\setminus\mathbb{R}_+.
\end{equation}
This allows us to leverage results from \citet{bigot2024high}, which provide the same definition. We note that
\begin{equation}
    \mathbb{E}\!\left[
\beta^{*\top}
M (X^\top X + \lambda M)^{-2} M
\beta^*
\right]=\sum_{j=1}^m\mathbb{E}\!\left[\mu_j^2(Q(-\lambda)^2)_{jj}\mu_j^{-2}q(\mu_j)\right]
=\sum_{j=1}^m\mathbb{E}\!\left[(Q(-\lambda)^2)_{jj}q(\mu_j)\right].
\end{equation}
Notably,
\begin{equation}
    Q(z)^2=Q'(z):=\frac{\text{d}}{\text{d}z}Q(z).
\end{equation}

\citet{bigot2024high} define a diagonal system of equations
\begin{equation}
    t_j(z):=-\frac{1}{z\Big(1+\frac1n\sum_{i=1}^n\frac{\tilde{t}_i(z)}{\mu_j}\Big)},\\
    \tilde{t}_i(z):=-\frac{1}{z\Big(1+\frac1n\sum_{j=1}^m\frac{t_j(z)}{\mu_j}\Big)}.
\end{equation}
(This is given by equations (2.1)-(2.2) in \citet{bigot2024high}; note that they use a slightly different notation; in particular our $m$ is their $p$; furthermore, they use cell-wise second moments $\gamma_{FT}_{ij}^2$, a key simplification in our system is that $\gamma_{FT}_{ij}^2=1/\mu_j$.)

This allow us to define the scalar quantity
\begin{equation}
    \tilde{t}(z):=-\frac{1}{z\Big(1+\frac1n\sum_{j=1}^m\frac{t_j(z)}{\mu_j}\Big)}.
\end{equation}
We then simplify
\begin{equation}
    t_j(z)=-\frac{1}{z\Big(1+\frac{\tilde{t}(z)}{\mu_j}\Big)}.\label{eq:tj}
\end{equation}
We now compute
\begin{equation}
    \sum_{j=1}^m\frac{t_j(z)}{\mu_j}=-\frac{1}{z}\sum_{j=1}^m\frac{1}{\mu_j+\tilde{t}(z)}.
\end{equation}
This implies
\begin{equation}
    \tilde{t}(z)=-\frac{1}{z-\frac{1}{n}\sum_{j=1}^m\frac{1}{\mu_j+\tilde{t}(z)}},
\end{equation}
which is a scalar fixed-point equation. In the limit of $n\to\infty$, this equation converges to
\begin{equation}
    \tilde{t}(z)=-\frac{1}{z-\gamma_{FT}\mathbb{E}_\mu\left[\frac{1}{\mu+\tilde{t}(z)}\right]},
\end{equation}
which we note is related to Stieltjes transform of $P_{\mu}$,
\begin{equation}
    m_{\mu}(s):=\mathbb{E}\left[\frac{1}{\mu-s}\right].
\end{equation}
Specifically:
\begin{equation}
    \tilde{t}(z)=-\frac{1}{z-\frac{1}{\gamma_{FT}}\mu_s(-\tilde{t}(z))}.\label{t:fp}
\end{equation}

\citet{bigot2024high} then show that with probability one (see Theorem 3.1),
\begin{equation}
    \sum_{j=1}^mQ'(-\lambda)_{jj}q(\mu_j)=\sum_{j=1}^m(t_j'(-\lambda)q(\mu_j),
\end{equation}
as long as $q(\mu_j)$ is bounded.

We now express $t_j'(-\lambda)$. Define the scalar map
\begin{equation}
\Phi(z,\tilde t)
:= \tilde t + \frac{1}{z-\frac{1}{n}\sum_{k=1}^m \frac{1}{\mu_k+\tilde t}}.
\end{equation}
Then $\tilde t(z)$ is characterized by
\begin{equation}
\Phi\big(z,\tilde t(z)\big)=0.
\end{equation}
Let
\begin{align}
S(z) &:= \frac{1}{n}\sum_{k=1}^m \frac{1}{\mu_k+\tilde t(z)}, \label{eq:t1}\\
R(z) &:= \frac{1}{n}\sum_{k=1}^m \frac{1}{(\mu_k+\tilde t(z))^2}. \label{eq:t2}
\end{align}
Note that $S(z)$ and $R(z)$ are scalar functions of $z$ through $\tilde t(z)$.

Differentiate \eqref{eq:t1} with respect to $z$:
\[
\partial_z \Phi\big(z,\tilde t(z)\big)+\partial_{\tilde t}\Phi\big(z,\tilde t(z)\big)\,\tilde t'(z)=0.
\]
A direct calculation yields
\begin{align}
\partial_z \Phi\big(z,\tilde t(z)\big)
&= -\frac{1}{\big(z-S(z)\big)^2}, \\
\partial_{\tilde t}\Phi\big(z,\tilde t(z)\big)
&= 1-\frac{R(z)}{\big(z-S(z)\big)^2}. 
\end{align}
Therefore,
\begin{equation}
\tilde t'(z)
=
\frac{1}{\big(z-S(z)\big)^2-R(z)}. 
\end{equation}
Using the fixed point \eqref{t:fp}, we also have
\begin{equation}
z-S(z)=-\frac{1}{\tilde t(z)}, 
\end{equation}
and hence an equivalent form is
\begin{equation}
\tilde t'(z)
=
\frac{1}{\tilde t(z)^{-2}-R(z)}. 
\end{equation}

We now compute $t'_j(z)$.
Differentiate \eqref{eq:tj} with respect to $z$. Writing $a_j(z):=1+\tilde t(z)/\mu_j$, we have
$t_j(z)=-(z a_j(z))^{-1}$ and $a_j'(z)=\tilde t'(z)/\mu_j$, so
\begin{align}
t_j'(z)
&=
\frac{a_j(z)+z a_j'(z)}{z^2 a_j(z)^2} \notag\\
&=
\frac{1}{z^2\Big(1+\frac{\tilde t(z)}{\mu_j}\Big)}
+
\frac{\tilde t'(z)}{z\,\mu_j\Big(1+\frac{\tilde t(z)}{\mu_j}\Big)^2}.
\end{align}
Evaluating at $z=-\lambda$ gives
\begin{equation}
t_j'(-\lambda)
=
\frac{1}{\lambda^2\Big(1+\frac{\tilde t(-\lambda)}{\mu_j}\Big)}
-
\frac{\tilde t'(-\lambda)}{\lambda\,\mu_j\Big(1+\frac{\tilde t(-\lambda)}{\mu_j}\Big)^2}.
\end{equation}
Overall, this implies that the first (signal) contribution admits the deterministic-equivalent representation
\begin{align}
\frac{\lambda^2}{m}\,
\mathbb{E}\!\left[
\beta^{*\top}M(X^\top X+\lambda M)^{-2}M\beta^*
\right]
&=
\frac{\lambda^2}{m}\sum_{j=1}^m \mathbb{E}\!\left[\mu_j^2 q(\mu_j)\,(G_\lambda^2)_{jj}\right] \nonumber\\
&\approx
\frac{\lambda^2}{m}\sum_{j=1}^m \mathbb{E}\!\left[q(\mu_j)\,t_j'(-\lambda)\right].
\label{eq:signal-deq}
\end{align}

Substituting the analytic expression for $t_j'(-\lambda)$ yields
\begin{align}
\frac{\lambda^2}{m}\sum_{j=1}^m \mathbb{E}\!\left[q(\mu_j)\,t_j'(-\lambda)\right]
&=
\frac{\lambda^2}{m}\sum_{j=1}^m \mathbb{E}\!\left[
q(\mu_j)
\left\{
\frac{1}{\lambda^2\left(1+\frac{\tilde t(-\lambda)}{\mu_j}\right)}
-
\frac{\tilde t'(-\lambda)}{\lambda\,\mu_j\left(1+\frac{\tilde t(-\lambda)}{\mu_j}\right)^2}
\right\}
\right]\nonumber\\
&=
\frac{1}{m}\sum_{j=1}^m \mathbb{E}\!\left[
q(\mu_j)\,\frac{1}{1+\frac{\tilde t(-\lambda)}{\mu_j}}
\right]
-\lambda\,\tilde t'(-\lambda)\,
\frac{1}{m}\sum_{j=1}^m
\mathbb{E}\!\left[
q(\mu_j)\,\frac{1}{\mu_j\left(1+\frac{\tilde t(-\lambda)}{\mu_j}\right)^2}
\right]\nonumber\\
&=
\frac{1}{m}\sum_{j=1}^m \mathbb{E}\!\left[
q(\mu_j)\,\frac{\mu_j}{\mu_j+\tilde t(-\lambda)}
\right]
-\lambda\,\tilde t'(-\lambda)\,
\frac{1}{m}\sum_{j=1}^m
\mathbb{E}\!\left[
q(\mu_j)\,\frac{\mu_j}{\left(\mu_j+\tilde t(-\lambda)\right)^2}
\right].
\label{eq:signal-expanded}
\end{align}
In the proportional limit $m/n\to\gamma_{FT}$ and under i.i.d.\ $\mu_j$, the law of large numbers yields
\begin{equation}
\lim_{n\to\infty}
\frac{\lambda^2}{m}\,
\mathbb{E}\!\left[
\beta^{*\top}M(X^\top X+\lambda M)^{-2}M\beta^*
\right]
=
\mathbb{E}_\mu\!\left[
q(\mu)\,\frac{\mu}{\mu+\tilde t(-\lambda)}
\right]
-\lambda\,\tilde t'(-\lambda)\,
\mathbb{E}_\mu\!\left[
q(\mu)\,\frac{\mu}{\left(\mu+\tilde t(-\lambda)\right)^2}
\right].
\label{eq:signal-limit}
\end{equation}

\paragraph{Simplifying the variance (noise) contribution.}
For the second term, note the exact identity (with $G_\lambda=(X^\top X+\lambda M)^{-1}$)
\begin{align}
X^\top X\,G_\lambda^2
&=
\bigl((X^\top X+\lambda M)-\lambda M\bigr)G_\lambda^2
=
G_\lambda-\lambda M G_\lambda^2,
\label{eq:trace-identity}
\end{align}
and hence
\begin{align}
\frac{\sigma_0^2}{m}\,
\mathbb{E}\!\left[
\mathrm{Tr}\!\left(
X^\top X (X^\top X + \lambda M)^{-2}
\right)
\right]
&=
\frac{\sigma_0^2}{m}\,
\mathbb{E}\!\left[\mathrm{Tr}(G_\lambda)\right]
-
\frac{\sigma_0^2\lambda}{m}\,
\mathbb{E}\!\left[\mathrm{Tr}(M G_\lambda^2)\right].
\label{eq:var-decomp}
\end{align}

Using the reparametrization $\tilde X=XM^{-1/2}$ and $\tilde G_\lambda=(\tilde X^\top\tilde X+\lambda I)^{-1}$,
we have the exact trace equalities
\begin{equation}
\mathrm{Tr}(G_\lambda)=\mathrm{Tr}(M^{-1}\tilde G_\lambda),
\qquad
\mathrm{Tr}(M G_\lambda^2)=\mathrm{Tr}(M^{-1}\tilde G_\lambda^2),
\label{eq:trace-rescale}
\end{equation}
so that
\begin{align}
\frac{1}{m}\mathrm{Tr}(G_\lambda)
&=
\frac{1}{m}\sum_{j=1}^m \frac{1}{\mu_j}(\tilde G_\lambda)_{jj},
\label{eq:traceG-diag}\\
\frac{1}{m}\mathrm{Tr}(M G_\lambda^2)
&=
\frac{1}{m}\sum_{j=1}^m \frac{1}{\mu_j}(\tilde G_\lambda^2)_{jj}.
\label{eq:traceMG2-diag}
\end{align}
Invoking Theorem~3.1 of \citet{bigot2024high} with the bounded diagonal test matrix
$U=\mathrm{diag}(\mu_1^{-1},\dots,\mu_m^{-1})$,
we may replace $(\tilde G_\lambda)_{jj}$ and $(\tilde G_\lambda^2)_{jj}$ by $t_j(-\lambda)$ and $t_j'(-\lambda)$,
respectively, obtaining
\begin{align}
\frac{1}{m}\mathrm{Tr}(G_\lambda)
&\approx
\frac{1}{m}\sum_{j=1}^m \frac{1}{\mu_j}t_j(-\lambda),
\label{eq:traceG-deq}\\
\frac{1}{m}\mathrm{Tr}(M G_\lambda^2)
&\approx
\frac{1}{m}\sum_{j=1}^m \frac{1}{\mu_j}t_j'(-\lambda).
\label{eq:traceMG2-deq}
\end{align}
Using $t_j(-\lambda)=\bigl[\lambda\bigl(1+\tilde t(-\lambda)/\mu_j\bigr)\bigr]^{-1}
=\mu_j\big/\bigl(\lambda(\mu_j+\tilde t(-\lambda))\bigr)$, we obtain
\begin{equation}
\frac{1}{\mu_j}t_j(-\lambda)=\frac{1}{\lambda(\mu_j+\tilde t(-\lambda))}.
\label{eq:invmu-tj}
\end{equation}
Likewise, using the explicit expression for $t_j'(-\lambda)$,
\begin{equation}
\frac{1}{\mu_j}t_j'(-\lambda)
=
\frac{1}{\lambda^2(\mu_j+\tilde t(-\lambda))}
-\frac{\tilde t'(-\lambda)}{\lambda(\mu_j+\tilde t(-\lambda))^2}.
\label{eq:invmu-tjprime}
\end{equation}
Substituting \eqref{eq:invmu-tj}--\eqref{eq:invmu-tjprime} into \eqref{eq:var-decomp} shows that the two
$\mathbb{E}[1/(\mu+\tilde t)]$ contributions cancel, yielding
\begin{align}
\frac{\sigma_0^2}{m}\,
\mathbb{E}\!\left[
\mathrm{Tr}\!\left(
X^\top X (X^\top X + \lambda M)^{-2}
\right)
\right]
&\approx
\sigma_0^2\,\tilde t'(-\lambda)\,
\frac{1}{m}\sum_{j=1}^m \mathbb{E}\!\left[\frac{1}{(\mu_j+\tilde t(-\lambda))^2}\right].
\label{eq:variance-simplified}
\end{align}
In the proportional limit $m/n\to\gamma_{FT}$ and under i.i.d.\ $\mu_j$, the law of large numbers yields
\begin{equation}
\lim_{n\to\infty}
\frac{\sigma_0^2}{m}\,
\mathbb{E}\!\left[
\mathrm{Tr}\!\left(
X^\top X (X^\top X + \lambda M)^{-2}
\right)
\right]
=
\sigma_0^2\,\tilde t'(-\lambda)\,
\mathbb{E}_\mu\!\left[\frac{1}{\bigl(\mu+\tilde t(-\lambda)\bigr)^2}\right].
\label{eq:variance-limit}
\end{equation}

\paragraph{Final per-coordinate error expression (ridge).}
Combining \eqref{eq:signal-limit} and \eqref{eq:variance-limit}, we obtain the asymptotic per-coordinate error
\begin{align}
\mathcal E
&=
\mathbb{E}_\mu\!\left[
q(\mu)\,\frac{\mu}{\mu+\tilde t(-\lambda)}
\right]
-\lambda\,\tilde t'(-\lambda)\,
\mathbb{E}_\mu\!\left[
q(\mu)\,\frac{\mu}{\left(\mu+\tilde t(-\lambda)\right)^2}
\right]
+
\sigma_0^2\,\tilde t'(-\lambda)\,
\mathbb{E}_\mu\!\left[
\frac{1}{\left(\mu+\tilde t(-\lambda)\right)^2}
\right].
\label{eq:final-risk}
\end{align}
